Diffusion Probabilistic Models for Structured Node Classification

This paper studies structured node classification on graphs, where the predictions should consider dependencies between the node labels. In particular, we focus on solving the problem for partially labeled graphs where it is essential to incorporate the information in the known label for predicting the unknown labels. To address this issue, we propose a novel framework leveraging the diffusion probabilistic model for structured node classification (DPM-SNC). At the heart of our framework is the extraordinary capability of DPM-SNC to (a) learn a joint distribution over the labels with an expressive reverse diffusion process and (b) make predictions conditioned on the known labels utilizing manifold-constrained sampling. Since the DPMs lack training algorithms for partially labeled data, we design a novel training algorithm to apply DPMs, maximizing a new variational lower bound. We also theoretically analyze how DPMs benefit node classification by enhancing the expressive power of GNNs based on proposing AGG-WL, which is strictly more powerful than the classic 1-WL test. We extensively verify the superiority of our DPM-SNC in diverse scenarios, which include not only the transductive setting on partially labeled graphs but also the inductive setting and unlabeled graphs.

==> 3_background.tex <==
\section{Background}
\label{sec:method}

\subsection{Structured node classification}

%Structured node classification is a task that involves predicting node labels in a graph, while considering dependencies between nodes. This approach is especially beneficial when working with graph-structured data, where connections between nodes provide information for classification process. However, conventional GNNs ignore joint dependency between node labels, especially critical in semi-supervised settings.

%In the following, we consider learning on a graph $G$ with attributes $\bm{x}$ to predict targets $\bm{y}$. The graph $G=(\mathcal{V}, \mathcal{E})$ consists of a node set $\mathcal{V}$ and an edge set $\mathcal{E}$. In graph $G$, we predict targets $\bm{y}$ using attributes $\bm{x}$, assuming that the attributes and the targets are associated with nodes, i.e., $\bm{x}=\{x_{i}: i \in \mathcal{V}\}$ and $\bm{y} = \{y_{i}: i \in \mathcal{V}\}$. In semi-supervised settings, we consider training on a graph $G$ with attributes $\bm{x}$ having partially labeled targets $\bm{y}$, denoted by unobserved targets $\bm{y}_U$ and observed targets $\bm{y}_L$. 

Structured node classification is a task of predicting node labels in a graph, while considering the dependencies between nodes. Specifically, we consider learning on a graph $G$ with attributes $\bm{x}$ to predict targets $\bm{y}$. The graph $G=(\mathcal{V}, \mathcal{E})$ consists of a node set $\mathcal{V}$ and an edge set $\mathcal{E}$. We assume that the attributes and the targets are associated with nodes, i.e., $\bm{x}=\{x_{i}: i \in \mathcal{V}\}$ and $\bm{y} = \{y_{i}: i \in \mathcal{V}\}$. In semi-supervised settings, we consider partially labeled targets $\bm{y}$, denoted by unobserved targets $\bm{y}_U$ and observed targets $\bm{y}_L$. 

\subsection{Diffusion Probabilistic models}

Diffusion probabilistic models are latent variable models consisting of two processes: the forward process and the reverse process\citep{ho2020denoising}. Given the variable $\bm{y}$, the fixed forward diffusion process iteratively injects noise into the data until converging to a standard Gaussian distribution. Conversely, the reverse diffusion process aims to reconstruct the data from the standard Gaussian distribution.

\textbf{Forward process.} Given a data $\bm{y}^{(0)}=\bm{y}$ and the total diffusion steps $T$, forward process constructs a sequence of latent variables $\bm{y}^{(1)}, \ldots, \bm{y}^{(T)}$ using a fixed distribution $q(\cdot)$.
\begin{align*}
q(\bm{y}^{(1)}, \ldots, \bm{y}^{(T)} |\bm{y}^{(0)}) = \prod_{t=1}^{T}q(\bm{y}^{(t)}|\bm{y}^{(t-1)}),\quad q(\bm{y}^{(t)}|\bm{y}^{(t-1)}) = \mathcal{N}(\bm{y}^{(t)};\sqrt{\alpha_{t}}\bm{y}^{(t-1)},\beta_{t}\mathbf{I}),
\end{align*}
where $\mathbf{I}$ is an identity matrix, $\beta_{1},\ldots, \beta_{T}$ are fixed variance schedules, and $\alpha_{t} = 1-\beta_{t}$. The variance schedule is designed to promote $q(\bm{y}^{(T)} | \bm{y}^{(0)}) \approx \mathcal{N}(\bm{y}^{(T)} ; \mathbf{0}, \mathbf{I})$ by setting $\beta_t < \beta_{t+1}$ for $t=0,\ldots,T-1$ and $\beta_T =1$. %We provide a detailed variance scheduling method in \Cref{appx:architecture_diffusion}.


\textbf{Reverse process.} Given an initial sample $\bm{y}^{(T)}$ from $p(\bm{y}^{(T)})=\mathcal{N}(\bm{y}^{(T)};\mathbf{0},\mathbf{I})$, the reverse process gradually denoises the latent variables to the data distribution with a parameterized distribution $p_{\bm{\theta}}(\cdot)$. 
\begin{gather*}
p_{\bm{\theta}}(\bm{y}^{(0)},\ldots, \bm{y}^{(T-1)} |\bm{y}^{(T)}) = \prod_{t=1}^{T}p_{\bm{\theta}}(\bm{y}^{(t-1)}|\bm{y}^{(t)}),\quad p_{\bm{\theta}}(\bm{y}^{(t-1)}|\bm{y}^{(t)}) = \mathcal{N}(\bm{y}^{(t-1)};\bm{\mu}_{\bm{\theta}}(\bm{y}^{(t)}),\sigma_t^2\mathbf{I}),
\end{gather*}
where the denoised mean value $\bm{\mu}_{\bm{\theta}}(\cdot)$ of $\bm{y}^{(t-1)}$ is typically parameterized with a neural network. Here, the reverse process also can be conditioned on additional inputs $\bm{x}$ like class labels, or text prompts. Then, the denoised mean value is defined with the additional inputs likes $\bm{\mu}_{\bm{\theta}}(\bm{y}^{(t-1)},\bm{x})$. 

\textbf{Training objective.} Then, DPM is trained to maximize the variational lower bound of the log-likelihood $\log p_{\bm{\theta}}(\bm{y}^{(0)})$ which is simplified by Ho et., \citep{ho2020denoising} as follows:
\begin{align}
\label{eq:ddpm_loss}
\mathcal{L}= \sum^{T}_{t=1}\frac{1}{\sigma^{2}_{t}}\mathbb{E}_{q(\bm{y}^{(t)} |\bm{y}^{(0)})}[\lVert \bm{\mu}_{\bm{\theta}}(\bm{y}^{(t)})-\hat{\bm{\mu}}\rVert^{2}_{2}].
\end{align}
Here, $\hat{\bm{\mu}}$ denotes average of the conditional distribution $q(\bm{y}^{(t-1)}|\bm{y}^{(t)},\bm{y}^{(0})$ that can be computed in a closed form with the fixed parameters of the distribution $q(\cdot)$. In practice, this objective is further simplified by predicting residual from the mean value \citep{ho2020denoising}.

\textbf{Manifold-constrained sampling.} 
Manifold-constrained sampling is a method used to generate samples that lie on a lower-dimensional manifold within a high-dimensional space \citep{chung2022improving}. It ensures that the generated samples preserve the intrinsic structure and properties of the underlying data, resulting in more accurate and reliable representations.
% Why manifold-constrained sampling is good for DPM?
% Pargraph to be added

%\textbf{Deterministic inference.} We basically use a deterministic inference algorithm to create a unique prediction of labels required for evaluation. Recall that the reverse diffusion process of DPM can produce a diverse set of predictions, a single best guess is required for the classification problem.

%In order to evaluate our DPM-SNC, we set $\bm{y}^{(T)}$ to be a zero vector $\bm{0}$, which is the average of $p(\bm{y}^{(T)})=\mathcal{N}(\bm{y}^{(T)}; \bm{0}, \mathbf{I})$. Then for $t = T,\ldots, 1$, the reverse diffusion process deterministically reconstructs $\bm{y}^{(t-1)}$ from $\bm{y}^{(t)}$ as the average of $p_{\bm{\theta}}(\bm{y}^{(t-1)}|\bm{y}^{(t)})$. If the target is one-hot relaxation of discrete labels, we discretize the final prediction by choosing a dimension with maximum value. %\footnote{We further investigate the various inference schemes in \Cref{subsec:exp-analysis}.}


==> nips/resources/alg_ddpm.tex <==
\begin{algorithm}[tb]
   \caption{Fully-supervised training of DPM-GSP}
   \label{alg:ddpm_train}
\begin{algorithmic}[1]
   \STATE \textbf{Input:} Graph $G$, node attributes $\bm{x}$, and labels $\bm{y}$
   \STATE Sample $t\sim \text{Uniform}(1,\ldots,T)$
   \STATE Sample $\bm{y}^{(t)}\sim q(\bm{y}^{(t)}|\bm{y}^{(0)})$
   \STATE Compute $\mu_{\theta}(\bm{y}^{(t)})$ and $\hat{\mu}$
   \STATE Update $\theta$ to minimize $\frac{1}{\sigma^{2}_{t}}\| \bm{\mu}_{\bm{\theta}}(\bm{y}^{(t)})-\hat{\bm{\mu}}\|^{2}_{2}$
\end{algorithmic}
\end{algorithm}

%\begin{algorithm}[tb]
%   \caption{Sampling from DPM-GSP.}
%   \label{alg:ddpm_infer}
%\begin{algorithmic}
%   \STATE Input: Graph $G$, and node attributes $\bm{x}$
%    \STATE Sample $\bm{y}^{(T)} \sim p(\bm{y}^{(T)})$
%    \FOR{$t=T,T-1,\ldots,1$}
%    \STATE Compute $\mu_{\theta}(\bm{y}^{(t)})$ with \Cref{blabla}
%    \STATE Sample $\bm{y}^{(t-1)} \sim \mathcal{N}(\bm{y}^{(t-1)}|\mu_{\theta}(\bm{y}^{(t)}),\sigma_t^2\mathbf{I})$
%    \ENDFOR
%    \STATE \textbf{return} $\bm{y}^{(0)}$
%\end{algorithmic}
%\end{algorithm}

==> nips/resources/alg_transductive.tex <==
\setlength{\textfloatsep}{0.2cm}
\begin{algorithm}[tb]
%\small
\caption{Semi-supervised training of DPM-GSP}
\label{alg:transductive}
\begin{algorithmic}[1]
   \STATE \textbf{Input:} Graph $G$, attributes $\bm{x}$, and targets $\bm{y}_L$.
   % \# of sampled $\bm{y}_U$ $N_1$, and \# of epoch in maximization step $N_2$.
   %number of expectation steps $N_1$, and number of maximization steps $N_2$
   \STATE Train a mean-field GNN $p_{\phi}(\bm{y} | \bm{x}, G)$ on $\bm{y}_L$ and $G$.
   \STATE Initialize the buffer $\mathcal{B}$ with samples from $p_{\phi}(\bm{y}_{U} | \bm{x}, G)$.
   % trained on $\bm{y}_L$ using a cross-entropy loss
   \REPEAT
   \FOR[Expectation step]{$i=1,\ldots,N_1$}
   \STATE Get $\bm{y}_U \sim p_{\theta}(\bm{y}_U|\bm{y}_L,\bm{x},G)$ using \\
   manifold-constrained sampling.\hfill{\textit{$\triangleright$~\Cref{appx:msg}}}
   \STATE Update $\mathcal{B} \gets \mathcal{B} \cup \{ \bm{y}_U\}$.
    \STATE If $|\mathcal{B}| > K$, remove oldest entity from $\mathcal{B}$.
   \ENDFOR 
   \FOR[Maximization step]{$i=1,\ldots,N_2$}
   \STATE Sample $\bm{y}_U \sim \mathcal{B}$.
   \STATE Update $\theta$ to minimize $\mathcal{L}$ in \cref{eq:ddpm_loss} \\
   with $G$, $\bm{x}$, and $\bm{y}=\bm{y}_{L} \cup \bm{y}_{U}$.
   \ENDFOR
   \UNTIL{converged}
\end{algorithmic}
\end{algorithm}

==> nips/resources/fig_monte.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
\centering
\begin{subfigure}{0.8\linewidth}
\centering
\includegraphics[width=\textwidth]{example-image}
  \caption{}
\end{subfigure}\label{fig:monte_carlo_sampling}
\end{wrapfigure}


==> nips/resources/fig_step-vs-depth.tex <==
% \begin{wrapfigure}{r}{0.36\textwidth}
% \begin{wrapfigure}{r}{0.33\textwidth}
% \centering
%     % \setlength{\belowcaptionskip}{-20pt}
%     \vspace{-20pt}
%     \includegraphics[width=0.98\linewidth]{nips/resources/figures/steps_vs_depth_node.png}
%     \caption{Number of GNN layers vs. diffusion steps in accuracy}\label{fig:depth_vs_step}
% % \begin{subfigure}[t]{0.98\linewidth}
% %     \centering
% %     \scalebox{0.8}{
% %         \begin{tabular}{lcc}
% %         \toprule
% %         Methods                                & N-Acc & Time \\
% %         \midrule
% %         GCNII ($16$) & 00.0 \stdv{0.0} \\
% %         DPM-GSP ($10$) & 00.0 \stdv{0.0} \\
% %         GCNII ($64$) & 00.0 \stdv{0.0} \\
% %         DPM-GSP ($20$) & 00.0 \stdv{0.0} \\
% %         \bottomrule
% %         \end{tabular}
% %     }
% %     \caption{caption2}\label{tab:time_performance}
% % \end{subfigure}

% \end{wrapfigure}


\begin{wrapfigure}{r}{0.32\textwidth}
\begin{minipage}[t]{\linewidth}
\centering
\includegraphics[width=0.95\textwidth]{nips/resources/figures/accuracy_over_step.pdf}
   \caption{Accuracy for changes in diffusion steps.}\label{fig:acc_over_step}
\end{minipage}
\begin{minipage}[t]{\linewidth}
  \centering
  \includegraphics[width=0.95\textwidth]{nips/resources/figures/vs_GCNII.pdf}
  \caption{Accuracy with varying inference time.}\label{fig:vs_GCNII}
\end{minipage}
\vspace{-.2in}
\end{wrapfigure}

==> nips/resources/fig_synthetic.tex <==
%\begin{wrapfigure}{r}{0.46\textwidth}
%\centering
%\begin{subfigure}[t]{0.48\linewidth}
%  \includegraphics[width=\textwidth]{nips/resources/figures/synthetic_true.pdf}
%  \caption{True labels}
%\end{subfigure}
%\centering
%\begin{subfigure}[t]{0.48\linewidth}
%  \includegraphics[width=\textwidth]{example-image}
%  \caption{GMNN (Acc$=$)}
%\end{subfigure}
%\centering
%\begin{subfigure}[t]{0.48\linewidth}
%  \includegraphics[width=\textwidth]{nips/resources/figures/synthetic_clgnn.pdf}
%  \caption{CLGNN ($87.5\%$)}
%\end{subfigure}
%\centering
%\begin{subfigure}[t]{0.48\linewidth}
%  \includegraphics[width=\textwidth]{nips/resources/figures/synthetic_dpm.pdf}
%  \caption{DPM-SNC ($98.5\%$)}
%\end{subfigure}
%\caption{green indicates labeled nodes (temporal)}
%\end{wrapfigure}

\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.19\linewidth}
  \includegraphics[width=\textwidth]{nips/resources/figures/synthetic_true.pdf}
  \caption{True labels}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.19\linewidth}
  \includegraphics[width=\textwidth]{nips/resources/figures/synthetic_gnn.pdf}
  \caption{GNN}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.19\linewidth}
  \includegraphics[width=\textwidth]{nips/resources/figures/synthetic_gmnn.pdf}
  \caption{GMNN}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.19\linewidth}
  \includegraphics[width=\textwidth]{nips/resources/figures/synthetic_clgnn.pdf}
  \caption{CLGNN}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.19\linewidth}
  \includegraphics[width=\textwidth]{nips/resources/figures/synthetic_dpm.pdf}
  \caption{DPM-SNC}
\end{subfigure}
\caption{The node classification on the graph, which is symmetric when known labels are ignored. The node color indicates the label. The green and red indicate the labeled nodes, and incorrectly classified nodes, respectively. In this graph, the GNN can not classify the node labels without considering dependencies with known labels. Our method, which considers the label dependencies in entire nodes, perfectly classifies all node labels.}\label{fig:synthetic_result}
\end{figure}



==> nips/resources/fig_synthetic_example.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
\centering
    %\setlength{\belowcaptionskip}{-22pt}
    \vspace{-.05in}
    \begin{subfigure}[t]{0.45\linewidth}
    \centering
        \includegraphics[width=0.95\linewidth]{nips/resources/figures/synthetic_true.pdf}
        \caption{Random}\label{subfig:first_synthetic}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\linewidth}
    \centering
        \includegraphics[width=0.95\linewidth]{nips/resources/figures/synthetic_true_type2.pdf}
        \caption{Cluster}\label{subfig:second_synthetic}
    \end{subfigure}
    \caption{Illustration of two scenarios. \sethlcolor{OliveGreen}\hl{Green} highlights known labels.}\label{fig:synthetic_scenario}
    \vspace{.35in}
\end{wrapfigure}

==> nips/resources/fig_vsGCNII_layer_time.tex <==
\begin{wrapfigure}{r}{0.33\textwidth}
\centering

    \setlength{\belowcaptionskip}{-22pt}
    \vspace{-12pt}
    \includegraphics[width=\linewidth] {nips/resources/figures/vs_GCNII.pdf}
    \caption{Accuracy with varying number of message passing}\label{fig:vs_GCNII}
%\begin{subfigure}[t]{\linewidth}
%    \includegraphics[width=\textwidth] {nips/resources/figures/vs_GCNII.pdf}
%    \caption{caption1}\label{fig:vs_GCNII}
%\end{subfigure}

% \begin{subfigure}[t]{0.98\linewidth}
%     \centering
%     \scalebox{0.8}{
%         \begin{tabular}{lcc}
%         \toprule
%         Methods                                & N-Acc & Time \\
%         \midrule
%         GCNII ($16$) & 00.0 \stdv{0.0} \\
%         DPM-GSP ($10$) & 00.0 \stdv{0.0} \\
%         GCNII ($64$) & 00.0 \stdv{0.0} \\
%         DPM-GSP ($20$) & 00.0 \stdv{0.0} \\
%         \bottomrule
%         \end{tabular}
%     }
%     \caption{caption2}\label{tab:time_performance}
% \end{subfigure}

\end{wrapfigure}

==> nips/resources/tab_classifier_free.tex <==
\begin{wraptable}{r}{0.45\textwidth}
\centering
\caption{blablabla}\label{tab:inference}
\scalebox{0.85}{
\begin{tabular}{lccc}
\toprule
Method & {Pubmed} & {Cora} & {Citeseer} \\
\midrule
Independent & & \\
Re-sample & & \\
MCG & & \\
\bottomrule
\end{tabular}
}
\end{wraptable}

==> nips/resources/tab_inductive2.tex <==
\begin{table*}[t]
\centering
\caption{The inductive node classification performance. N-Acc and G-Acc denote the node-level and graph-level accuracy, respectively. \textbf{Bold} numbers indicate the best performance among the structured prediction methods using the same GNN. \underline{Underlined} numbers indicate the best score.
}\label{tab:inductive}
\scalebox{0.83}{
\begin{tabular}{lccccccc}
\toprule
& \multicolumn{2}{c}{Pubmed} & \multicolumn{2}{c}{Cora} & \multicolumn{2}{c}{Citeseer} & PPI \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7} \cmidrule(lr){8-8} 
Method & \multicolumn{1}{c}{N-Acc} & \multicolumn{1}{c}{G-Acc} & \multicolumn{1}{c}{N-Acc} & \multicolumn{1}{c}{G-Acc} & \multicolumn{1}{c}{N-Acc} & \multicolumn{1}{c}{G-Acc} & F1 \\
\midrule
GCN & 80.25 \stdv{0.42} & 54.58 \stdv{0.51} & 83.36 \stdv{0.43} & 59.67 \stdv{0.51} & 76.37 \stdv{0.35} & 49.84 \stdv{0.47} & 99.15 \stdv{0.03} \\
$+$G3NN & 80.32 \stdv{0.30} & 53.93 \stdv{0.71} & 83.60 \stdv{0.25} & 59.78 \stdv{0.47} & 76.34 \stdv{0.37} & 50.76 \stdv{0.47} & 99.33 \stdv{0.02}\\
$+$CLGNN & 80.22 \stdv{0.45} & 53.98 \stdv{0.54} & 83.45 \stdv{0.34} & 60.24 \stdv{0.38} & 75.71 \stdv{0.40} & 50.51 \stdv{0.38} & 99.22 \stdv{0.04} \\
$+$SPN & \underline{\textbf{80.78}} \stdv{0.34} & 54.91 \stdv{0.40} & 83.85 \stdv{0.60} & 60.35 \stdv{0.57} & 76.25 \stdv{0.48} & 51.02 \stdv{1.06} & 99.35 \stdv{0.02} \\
$+$DPM-GSP & {80.68} \stdv{0.41} & \underline{\textbf{55.16}} \stdv{0.43} & \underline{\textbf{84.09}} \stdv{0.27} & \underline{\textbf{60.88}} \stdv{0.36} & \underline{\textbf{77.01}} \stdv{0.49} & \textbf{51.44} \stdv{0.56} & \textbf{99.46} \stdv{0.02}\\
%$+$DPM-GSP$^{\ast}$ &  \\
\midrule
GraphSAGE & 79.62 \stdv{0.76} & {53.49} \stdv{0.76} & {81.55} \stdv{0.48} & {57.83} \stdv{0.63} & {74.23} \stdv{0.88} & {47.94} \stdv{1.09} & 99.48 \stdv{0.02}\\
$+$G3NN & \textbf{79.83} \stdv{1.55} & 52.98 \stdv{0.90} & 81.62 \stdv{0.31} & 58.31 \stdv{0.59} & 74.70 \stdv{0.67} & 48.38 \stdv{0.61} & 99.49 \stdv{0.01}\\
$+$CLGNN & 78.98 \stdv{0.56} & 53.42 \stdv{0.42} & 82.49 \stdv{0.33} & 59.04 \stdv{0.70} & 74.72 \stdv{0.92} & 48.55 \stdv{1.16} &  99.50 \stdv{0.02} \\
$+$SPN & 79.55 \stdv{1.15} & \textbf{54.03} \stdv{0.71} & 82.31 \stdv{0.48} & \textbf{59.58} \stdv{1.30} & 75.83 \stdv{0.68} & 50.81 \stdv{1.18} & 99.51 \stdv{0.02}\\
$+$DPM-GSP & 79.43 \stdv{0.80} & 53.75 \stdv{0.68} & \textbf{83.06} \stdv{0.37} & {59.55} \stdv{0.88} & \textbf{76.58} \stdv{0.67} & \textbf{51.66} \stdv{0.69} & \textbf{99.62} \stdv{0.03} \\
%$+$DPM-GSP$^{\ast}$ &  \\
\midrule
GAT & 80.10 \stdv{0.45} & 54.38 \stdv{0.54} & 79.71 \stdv{1.41} & 56.66 \stdv{1.40} & 74.91 \stdv{0.22} & 49.87 \stdv{0.44} & 99.54 \stdv{0.01} \\
$+$G3NN & 79.88 \stdv{0.62} & 54.66 \stdv{0.29} & 81.19 \stdv{0.45} & 58.68 \stdv{0.38} & 75.45 \stdv{0.26} & 50.86 \stdv{0.46} & 99.56 \stdv{0.01} \\
$+$CLGNN & 80.23 \stdv{0.40} & 54.51 \stdv{0.36} & 81.38 \stdv{0.55} & {58.81} \stdv{0.61} & 75.45 \stdv{0.36} & 50.66 \stdv{0.45} & 99.55 \stdv{0.01}\\
$+$SPN & 79.95 \stdv{0.34} & \textbf{54.82} \stdv{0.33} & 81.61 \stdv{0.31} & 59.17 \stdv{0.31} & 75.41 \stdv{0.35} & 51.04 \stdv{0.53} & 99.46 \stdv{0.02}\\
$+$DPM-GSP & \textbf{80.26} \stdv{0.37} & 54.26 \stdv{0.47} & \textbf{81.79} \stdv{0.46} & \textbf{59.55} \stdv{0.49} & \textbf{76.46} \stdv{0.60} & \underline{\textbf{52.05}} \stdv{0.71} & \underline{\textbf{99.63}} \stdv{0.01} \\
%$+$DPM-GSP$^{\ast}$ &  \\
\bottomrule
\end{tabular}
}
\end{table*}


==> nips/resources/tab_inductive_huge.tex <==
\begin{table*}[h]
\centering
\caption{The inductive node classification performance. N-Acc denotes the node-level accuracy. \textbf{Bold} numbers indicate the best performance among the structured prediction methods using the same GNN. \underline{Underlined} numbers indicate the best performance.}\label{tab:inductive_huge}
%\resizebox{\textwidth}{!}{% 
%\begin{tabular}{llcc@{\hspace{5pt}}cc@{\hspace{5pt}}cc@{\hspace{5pt}}cc@{\hspace{5pt}}c}
\scalebox{0.8}{
\begin{tabular}{l@{\hspace{10pt}}c@{\hspace{8pt}}c@{\hspace{10pt}}c@{\hspace{8pt}}c@{\hspace{10pt}}c@{\hspace{8pt}}c@{\hspace{10pt}}c@{\hspace{8pt}}c}
\toprule
& \multicolumn{2}{c}{PPI-1} & \multicolumn{2}{c}{PPI-2} & \multicolumn{2}{c}{PPI-10} & \multicolumn{2}{c}{PPI-20}\\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
Method & \multicolumn{1}{c}{N-Acc} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{N-Acc} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{N-Acc} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{N-Acc} & \multicolumn{1}{c}{F1}\\
\midrule
GCN & 80.85 \stdv{0.22} & 65.08 \stdv{0.39} & 83.16 \stdv{0.14} & 71.67 \stdv{0.22} & 97.74 \stdv{0.03} & 96.16 \stdv{0.03} & 99.15 \stdv{0.03} & 98.57 \stdv{0.05} \\ 
$+$G3NN &  81.57 \stdv{0.19} & 66.15 \stdv{0.27} & 83.74 \stdv{0.10} & 72.07 \stdv{0.20} & 97.84 \stdv{0.04} & 96.30 \stdv{0.06} & 99.33 \stdv{0.02} & 98.88 \stdv{0.01} \\
$+$CLGNN & 81.42 \stdv{0.24} & 66.02 \stdv{0.42} & 83.47 \stdv{0.17} & 71.82 \stdv{0.33} & 97.81 \stdv{0.03} & 96.28 \stdv{0.04} & 99.22 \stdv{0.04} & 98.62 \stdv{0.04} \\
$+$SPN & 81.93 \stdv{0.43} & 68.12 \stdv{0.19} & 85.42 \stdv{0.34} & 74.05 \stdv{0.15} & 97.57 \stdv{0.07} & 95.34 \stdv{0.14} & 99.35 \stdv{0.02} & 98.65 \stdv{0.03} \\
$+$DPM-GSP  & \textbf{83.77} \stdv{0.27} & \textbf{70.08} \stdv{0.43} & \textbf{86.63} \stdv{0.24} & \textbf{76.20} \stdv{0.43} & \textbf{98.21} \stdv{0.08} & \textbf{97.00} \stdv{0.09} & \textbf{99.46} \stdv{0.02} & \textbf{99.02} \stdv{0.02} \\
%$+$DPM-GSP$^{\ast}$ & \\
\midrule
GraphSAGE & 79.88 \stdv{0.36} & 65.13 \stdv{0.42} & 83.04 \stdv{0.27} & 70.87 \stdv{0.29} & 97.33 \stdv{0.06} & 95.55 \stdv{0.09} & 99.48 \stdv{0.02} & 99.14 \stdv{0.03} \\
$+$G3NN & 80.66 \stdv{0.23} & 66.48 \stdv{0.31} & 84.15 \stdv{0.15} & 73.24 \stdv{0.23} & 97.52 \stdv{0.06} & 95.85 \stdv{0.04} & 99.49 \stdv{0.01} & 99.14 \stdv{0.02} \\
$+$CLGNN & 80.13 \stdv{0.19} & 65.89 \stdv{0.42} & 84.09 \stdv{0.32} & 71.69 \stdv{0.18} & 97.79 \stdv{0.04} & 96.24 \stdv{0.06} & 99.50 \stdv{0.02} & 99.17 \stdv{0.03}\\
$+$SPN & 81.84 \stdv{0.41} & 68.02 \stdv{0.20} & 85.88 \stdv{0.22} & 74.92 \stdv{0.11} & 97.93 \stdv{0.06} & 96.12 \stdv{0.09} & 99.51 \stdv{0.02} & 99.15 \stdv{0.04} \\
$+$DPM-GSP  & \underline{\textbf{83.96}} \stdv{0.14} & \underline{\textbf{70.90}} \stdv{0.41} & \underline{\textbf{87.49}} \stdv{0.19} & \underline{\textbf{78.20}} \stdv{0.35} & \underline{\textbf{98.36}} \stdv{0.03} & \underline{\textbf{97.20}} \stdv{0.05} & \textbf{99.62} \stdv{0.03} & \underline{\textbf{99.30}} \stdv{0.03} \\
%+$DPM-GSP$^{\ast}$ & \\
\midrule
GAT & 78.25 \stdv{0.33} & 63.88 \stdv{0.75} & 81.06 \stdv{0.24} & 69.62 \stdv{0.34} & 98.07 \stdv{0.07} & 96.65 \stdv{0.13} & 99.54 \stdv{0.01} & 99.23 \stdv{0.02} \\
$+$G3NN & 79.16 \stdv{0.38} & 64.25 \stdv{0.53} & 82.57 \stdv{0.28} & 71.07 \stdv{0.29} & 98.22 \stdv{0.04} & 96.81 \stdv{0.04} & 99.56 \stdv{0.01} & 99.26 \stdv{0.01} \\
$+$CLGNN & 79.00 \stdv{0.22} & 64.17 \stdv{0.46} & 83.04 \stdv{0.18} & 71.50 \stdv{0.36} & 98.14 \stdv{0.05} & 96.77 \stdv{0.10} & 99.55 \stdv{0.01} & 99.24 \stdv{0.02} \\
$+$SPN & 80.29 \stdv{0.31} & 64.72 \stdv{0.20} & 84.79 \stdv{0.47} & 73.07 \stdv{0.22} & 97.80 \stdv{0.08} & 96.06 \stdv{0.04} & 99.46 \stdv{0.02} & 99.11 \stdv{0.03} \\
$+$DPM-GSP  & \textbf{81.94} \stdv{0.24} & \textbf{66.83} \stdv{0.32} & \textbf{86.43} \stdv{0.15} & \textbf{75.82} \stdv{0.24} & \textbf{98.30} \stdv{0.07} & \textbf{97.06} \stdv{0.10} & \underline{\textbf{99.63}} \stdv{0.01} & \underline{\textbf{99.30}} \stdv{0.01} \\
%$+$DPM-GSP$^{\ast}$ &  \\
\bottomrule
 \end{tabular}}
\end{table*}



==> nips/resources/tab_inductive_small.tex <==
\begin{table*}[t]
\centering
\caption{The inductive node classification accuracy. N-Acc and G-Acc denote the node-level and graph-level accuracy, respectively. \textbf{Bold} numbers indicate the best performance among the structured prediction methods using the same GNN. \underline{Underlined} numbers indicate the best performance.
}\label{tab:inductive_small}
\scalebox{0.8}{
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{Pubmed} & \multicolumn{2}{c}{Cora} & \multicolumn{2}{c}{Citeseer} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
Method & \multicolumn{1}{c}{N-Acc} & \multicolumn{1}{c}{G-Acc} & \multicolumn{1}{c}{N-Acc} & \multicolumn{1}{c}{G-Acc} & \multicolumn{1}{c}{N-Acc} & \multicolumn{1}{c}{G-Acc}\\
\midrule
GCN & 80.25 \stdv{0.42} & 54.58 \stdv{0.51} & 83.36 \stdv{0.43} & 59.67 \stdv{0.51} & 76.37 \stdv{0.35} & 49.84 \stdv{0.47} \\
$+$G3NN & 80.32 \stdv{0.30} & 53.93 \stdv{0.71} & 83.60 \stdv{0.25} & 59.78 \stdv{0.47} & 76.34 \stdv{0.37} & 50.76 \stdv{0.47} \\
$+$CLGNN & 80.22 \stdv{0.45} & 53.98 \stdv{0.54} & 83.45 \stdv{0.34} & 60.24 \stdv{0.38} & 75.71 \stdv{0.40} & 50.51 \stdv{0.38} \\
$+$SPN & 80.39 \stdv{0.34} & 54.68 \stdv{0.40} & 83.85 \stdv{0.60} & 60.35 \stdv{0.57} & 76.25 \stdv{0.48} & 51.02 \stdv{1.06} \\
$+$DPM-GSP & \underline{\textbf{80.68}} \stdv{0.41} & \underline{\textbf{55.16}} \stdv{0.43} & \textbf{84.09} \stdv{0.27} & \textbf{60.88} \stdv{0.36} & \underline{\textbf{77.01}} \stdv{0.49} & \textbf{51.44} \stdv{0.56} \\
%$+$DPM-GSP$^{\ast}$ &  \\
\midrule
GraphSAGE & 79.62 \stdv{0.76} & {53.49} \stdv{0.76} & {81.55} \stdv{0.48} & {57.83} \stdv{0.63} & {74.23} \stdv{0.88} & {47.94} \stdv{1.09} \\
$+$G3NN & \textbf{79.83} \stdv{1.55} & 52.98 \stdv{0.90} & 81.62 \stdv{0.31} & 58.31 \stdv{0.59} & 74.70 \stdv{0.67} & 48.38 \stdv{0.61} \\
$+$CLGNN & 78.98 \stdv{0.56} & 53.42 \stdv{0.42} & 82.49 \stdv{0.33} & 59.04 \stdv{0.70} & 74.72 \stdv{0.92} & 48.55 \stdv{1.16} \\
$+$SPN & 79.55 \stdv{1.15} & \textbf{54.03} \stdv{0.71} & 82.31 \stdv{0.48} & 59.58 \stdv{1.30} & 75.83 \stdv{0.68} & 50.81 \stdv{1.18} \\
$+$DPM-GSP & 79.43 \stdv{0.80} & 53.75 \stdv{0.68} & \textbf{83.63} \stdv{0.27} & \textbf{60.06} \stdv{0.81} & \textbf{76.58} \stdv{0.67} & \textbf{51.66} \stdv{0.69} \\
%$+$DPM-GSP$^{\ast}$ &  \\
\midrule
GAT & 80.10 \stdv{0.45} & 54.38 \stdv{0.54} & 83.52 \stdv{0.69} & 59.07 \stdv{0.75} & 74.91 \stdv{0.22} & 49.87 \stdv{0.44} \\
$+$G3NN & 79.88 \stdv{0.62} & 54.66 \stdv{0.29} & 83.58 \stdv{0.45} & 60.91 \stdv{0.45} & 75.45 \stdv{0.26} & 50.86 \stdv{0.46} \\
$+$CLGNN & 80.23 \stdv{0.40} & 54.51 \stdv{0.36} & 83.96 \stdv{0.20} & \underline{\textbf{61.50}} \stdv{0.82} & 75.45 \stdv{0.36} & 50.66 \stdv{0.45} \\
$+$SPN & \textbf{80.38} \stdv{0.34} & \textbf{54.82} \stdv{0.33} & 83.80 \stdv{0.61} & 60.69 \stdv{0.94} & 75.41 \stdv{0.35} & 51.04 \stdv{0.53} \\
$+$DPM-GSP & 80.26 \stdv{0.37} & 54.66 \stdv{0.47} & \underline{\textbf{84.61}} \stdv{0.57} & 61.04 \stdv{0.72} & \textbf{76.46} \stdv{0.60} & \underline{\textbf{52.05}} \stdv{0.71} \\
%$+$DPM-GSP$^{\ast}$ &  \\
\bottomrule
\end{tabular}
}
\end{table*}



==> nips/resources/tab_inference.tex <==
\begin{wraptable}{r}{0.45\textwidth}
\centering
\caption{blablabla}\label{tab:inference}
\scalebox{0.85}{
\begin{tabular}{lccc}
\toprule
Method & {Pubmed} & {Cora} & {Citeseer} \\
\midrule
Independent & & \\
Re-sample & & \\
Manifold-constrained & & \\
\bottomrule
\end{tabular}
}
\end{wraptable}

==> nips/resources/tab_noising.tex <==
\begin{table*}[t]
\centering
\caption{The inductive node classification accuracy. N-Acc and G-Acc denote the node-level and graph-level accuracy, respectively. The backbone network is GAT. The Gaussian diffusion process outperforms the considered baselines specialized to discrete label.}\label{tab:noising}
%\resizebox{\linewidth}{!}{
\scalebox{0.8}{
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{PPI-1} & \multicolumn{2}{c}{Connected components} & \multicolumn{2}{c}{Citeseer} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
Method & N-Acc & G-Acc & N-Acc & G-Acc & N-Acc & G-Acc\\
\midrule
Absorbing & 79.08 \stdv{0.86} & 53.45 \stdv{0.48} & 81.66 \stdv{1.40} & 55.34 \stdv{1.49} & 74.22 \stdv{0.84} & 49.37 \stdv{1.11} \\
Uniform & 70.78 \stdv{0.89} & 38.79 \stdv{1.16} & 63.26 \stdv{0.82} & 25.88 \stdv{1.08} & 57.05 \stdv{0.61} & 22.51 \stdv{1.22} \\
Bit-upscale & 79.42 \stdv{0.79} & 53.92 \stdv{0.27} & 82.62 \stdv{0.32} & 56.25 \stdv{0.42} & 75.51 \stdv{0.58} & 51.19 \stdv{0.80} \\
Gaussian & \textbf{79.89} \stdv{0.26} & \textbf{54.60} \stdv{0.48} & \textbf{84.36} \stdv{0.59} & \textbf{60.15} \stdv{0.51} & \textbf{76.20} \stdv{0.65} & \textbf{52.03} \stdv{0.90} \\
\bottomrule
\end{tabular}
}
\end{table*}



==> nips/resources/tab_time_performance.tex <==
\begin{wraptable}{r}{0.45\textwidth}
\caption{ 
}\label{tab:time}
\centering
\scalebox{0.8}{
\centering
\begin{tabular}{lccc}
\toprule
& \multicolumn{3}{c}{Citeseer} \\
\cmidrule(lr){2-4}
Methods                                & N-Acc & Sub-Acc              & Time \\
\midrule
GCNII ($16$) & 00.0 \stdv{0.0} & 00.0 \stdv{0.0}  & 00.0     \\
DPM-GSP ($20$) & 00.0 \stdv{0.0} & 00.0 \stdv{0.0} & 00.0 \\
GCNII ($64$) & 00.0 \stdv{0.0} & 00.0 \stdv{0.0}  & 00.0     \\
DPM-GSP ($80$) & 00.0 \stdv{0.0} & 00.0 \stdv{0.0} & 00.0 \\
\bottomrule
\end{tabular}
}
\end{wraptable}

==> nips/resources/tab_transductive2.tex <==
\begin{table}[h]
\centering
\caption{The transductive node classification accuracy for homophily graphs. \textbf{Bold} numbers indicate the best performance among the structured prediction methods using the same GNN. \underline{Underlined} numbers indicate the best performance. 
}\label{tab:transductive}
\scalebox{0.8}{
\begin{tabular}{l@{\hspace{10pt}}c@{\hspace{5pt}}c@{\hspace{8pt}}c@{\hspace{5pt}}c@{\hspace{8pt}}c@{\hspace{5pt}}c@{\hspace{8pt}}c@{\hspace{5pt}}c@{\hspace{8pt}}c@{\hspace{5pt}}c}
\toprule
& \multicolumn{2}{c}{Pubmed} & \multicolumn{2}{c}{Cora} & \multicolumn{2}{c}{Citeseer} & \multicolumn{2}{c}{Photo} & \multicolumn{2}{c}{Computer} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
Method & N-Acc & Sub-Acc & N-Acc & Sub-Acc & N-Acc & Sub-Acc & N-Acc & Sub-Acc & N-Acc & Sub-Acc\\
\midrule
GCN & 79.7 \stdv{0.3} & 55.8 \stdv{0.6} & 81.4 \stdv{0.8} & 60.0 \stdv{0.6} & 71.1 \stdv{0.8} & 51.3 \stdv{0.6} & 91.0 \stdv{1.2} & 52.0 \stdv{1.0} & 82.8 \stdv{1.2} & 26.6 \stdv{1.5}  \\ 
$+$ GMNN & 82.6 \stdv{0.5} & 58.5 \stdv{0.9} & 82.1 \stdv{0.7} & 62.1 \stdv{1.0} & 72.2 \stdv{0.7} & 51.4 \stdv{0.8} & 91.6 \stdv{1.0} & 54.3 \stdv{1.4} & 83.1 \stdv{2.0} & 29.1 \stdv{1.8} \\
$+$ G3NN & 80.9 \stdv{0.7} & 56.9 \stdv{1.1} & 82.2 \stdv{0.3} & 62.1 \stdv{0.7} & 73.9 \stdv{0.7} & 53.1 \stdv{1.0} & 90.7 \stdv{1.1} & 53.0 \stdv{2.0} & 82.1 \stdv{1.2} & 28.1 \stdv{2.1} \\
$+$ CLGNN & 81.6 \stdv{0.7} & 58.0 \stdv{0.8} & 81.9 \stdv{0.7} & 61.8 \stdv{0.8} & 71.9 \stdv{0.8} & 52.1 \stdv{1.2} & 91.1 \stdv{1.0} & 53.4 \stdv{1.8} & 83.5 \stdv{1.2} &  28.9 \stdv{1.6}\\
$+$ DPM-GSP & \underline{\textbf{83.0}} \stdv{0.9} & \textbf{59.2} \stdv{1.2} & \textbf{83.0} \stdv{0.5} & \textbf{63.0} \stdv{0.9} & \underline{\textbf{74.4}} \stdv{0.5} & \textbf{53.6} \stdv{0.6} & \textbf{92.2} \stdv{0.8} & \textbf{55.3} \stdv{2.1} & \textbf{84.1} \stdv{1.3} & \textbf{30.0} \stdv{1.8} \\
\midrule
SAGE & 76.8 \stdv{0.8} & 53.2 \stdv{0.9} & 80.2 \stdv{0.7} & 57.6 \stdv{0.5} & 70.9 \stdv{1.0} & 48.9 \stdv{0.5} & 91.3 \stdv{0.9} & 49.8 \stdv{1.9} & 82.1 \stdv{0.9} & 25.4 \stdv{1.3}  \\ 
$+$ GMNN & 78.2 \stdv{1.2} & 56.5 \stdv{1.6} & 81.2 \stdv{0.8} & 60.9 \stdv{1.1} & 71.6 \stdv{0.9} & 51.2 \stdv{0.7} & 91.5 \stdv{1.1} & 52.5 \stdv{1.4} & 82.9 \stdv{2.4} & 26.9 \stdv{1.8} \\
$+$ G3NN & 78.4 \stdv{1.1} & 56.1 \stdv{1.3} & 82.0 \stdv{0.6} & 61.4 \stdv{1.0} & \textbf{72.9} \stdv{0.5} & \textbf{52.2} \stdv{0.8} & 91.0 \stdv{1.6} & 52.1 \stdv{3.0} & {83.0} \stdv{2.0} & 26.6 \stdv{2.0} \\
$+$ CLGNN & 77.2 \stdv{1.1} & 55.8 \stdv{1.4} & 80.8 \stdv{0.4} & 59.0 \stdv{0.8} & 71.5 \stdv{0.8} & 51.0 \stdv{1.0} & 91.4 \stdv{0.8} &  51.6 \stdv{2.1} & 83.4 \stdv{1.2} &  27.1 \stdv{1.6}\\
$+$ DPM-GSP & \textbf{79.7} \stdv{1.3} & \textbf{58.1} \stdv{1.0} & \textbf{82.8} \stdv{0.7} & \textbf{62.2} \stdv{1.0} & {72.4} \stdv{0.7} & {51.7} \stdv{0.9} & \underline{\textbf{92.3}} \stdv{0.7} & \textbf{53.2} \stdv{2.2} & \textbf{83.9} \stdv{1.5} & \textbf{28.1} \stdv{1.6}\\
%$+$ DPM-GSP$^{\ast}$ &  \\
\midrule 
GAT & 79.1 \stdv{0.5} & 55.8 \stdv{0.5} & 81.5 \stdv{0.6} & 61.3 \stdv{0.9} & 71.3 \stdv{0.8} & 51.2 \stdv{1.0} & 91.2 \stdv{1.2} & 51.1 \stdv{1.9} & 83.4 \stdv{1.3} & 28.8 \stdv{1.7}  \\ 
$+$ GMNN & 80.9 \stdv{0.4} & 58.7 \stdv{0.8} & 82.3 \stdv{0.7} & 62.0 \stdv{1.0} & 71.7 \stdv{0.7} & 51.5 \stdv{0.8} & 91.6 \stdv{1.0} & 54.3 \stdv{1.4} & 83.1 \stdv{2.0} & 29.1 \stdv{1.8} \\
$+$ G3NN & 77.9 \stdv{0.4} & 55.9 \stdv{0.5} & 82.7 \stdv{1.3} & 62.7 \stdv{1.3} & {74.0} \stdv{0.8} & 53.7 \stdv{0.5} & 91.5 \stdv{0.9} &  52.6 \stdv{2.2} & 83.1 \stdv{1.7} & 28.8 \stdv{2.4} \\
$+$ CLGNN & 80.0 \stdv{0.6} & 58.3 \stdv{1.2} & 82.0 \stdv{0.9} & 61.5 \stdv{0.9} & 71.6 \stdv{0.7} & 51.6 \stdv{0.8} & 90.8 \stdv{1.1} & 51.9 \stdv{1.8} & 83.6 \stdv{1.2} & 29.0 \stdv{2.0}\\
$+$ DPM-GSP & \textbf{82.0} \stdv{0.2} & \textbf{59.7} \stdv{0.6} & \underline{\textbf{83.5}} \stdv{0.7} & \textbf{63.5} \stdv{0.7} & \textbf{74.3} \stdv{0.7} & \textbf{54.0} \stdv{0.9} & \textbf{92.0} \stdv{0.8} & \textbf{54.0} \stdv{2.4} & \underline{\textbf{84.5}} \stdv{1.5} & \textbf{30.1} \stdv{2.5} \\
%$+$ DPM-GSP$^{\ast}$ &  \\
\bottomrule
 \end{tabular}
}
\end{table}

